Efficient Community Detection in Boolean Composed Multiplex Networks

Networks (or graphs) are used to model the dyadic relations between entities in a complex system. In cases where there exists multiple relations between the entities, the complex system can be represented as a multilayer network, where the network in each layer represents one particular relation (or feature). The analysis of multilayer networks involves combining edges from specific layers and then computing a network property. Different subsets of the layers can be combined. For any Boolean combination operation (e.g. AND, OR), the number of possible subsets is exponential to the number of layers. Thus recomputing for each subset from scratch is an expensive process. In this paper, we propose to efficiently analyze multilayer networks using a method that we term network decomposition. Network decomposition is based on analyzing each network layer individually and then aggregating the analysis results. We demonstrate the effectiveness of using network decomposition for detecting communities on different combinations of network layers. Our results on multilayer networks obtained from real-world and synthetic datasets show that our proposed network decomposition method requires significantly lower computation time while producing results of high accuracy.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

==> texFiles/BooleanExpression.tex <==
\section{Processing Boolean Expressions for Composed Layer Communities}
\label{sec:BooleanExpression}

==> texFiles/case_studies.tex <==
\section{Case Studies}
\label{sec:case-studies}

==> texFiles/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> texFiles/experiments.tex <==
\section{Experimental Analysis}
\label{sec:experiments}

==> texFiles/experiments_OR.tex <==
\section{Experimental Analysis (OR Composition)}
\label{sec:experiments-OR}

Experimental setup and MLNs (IMDB, DBLP, Accident, RMat) used for OR Composition are same as AND Composition experiments discussed in Section \ref{sec:experiments-AND}.

\begin{figure}[h]
    \centering
  \includegraphics[width=\linewidth]{./figures/OR-accuracy-v1}
    \caption{Accuracy Results of CE-OR Approach}
    \label{fig:OR-acc}  
\end{figure}

\noindent\textbf{Accuracy Results: } Similar to AND compositions, a total of 4 OR-Compositions are possible (3 2-layer and 1 3-layer). Communities obtained using the C-SG-OR are used as ground truth for each composition. Figure \ref{fig:AND-acc} shows that with respect to NMI and m-NMI, the \textbf{overall accuracy of the set of communities obtained with the two weight metrics (Aggregate and  Fraction) is at least 70\% for different MLNs}.


%\noindent\textbf{Cost Analysis:} In general for decoupling based approaches, the cost of the decoupling approach can be broken down into \textit{one time cost} (that is the time to find layer-wise communities) and cost of combining the partial results.

\begin{figure}[h]
    \centering
  \includegraphics[width=\linewidth]{./figures/OR-eff-v1}
    \caption{Efficiency of CE-OR as compared to C-SG-OR}
    \label{fig:OR-time}
\end{figure}

\noindent\textbf{Cost Analysis:} For CE-OR, CV-AND is used as a subroutine. Moreover, one scan of \textit{community edges} is required to generate the meta graph (OR-MG) on which we apply Infomap to generate communities. Clearly, if the layer densities are low (sparse layers), then cost of generating the meta graph and applying Infomap will become an overhead as compared to applying Infomap on OR graph (C-SG-OR approach). This can be seen from the DBLP MLN where sparse layers (density of densest layer (SIGMOD) = 0.0001!) make the CE-OR 67\% less efficient as compared to C-SG-OR. However, \textbf{for MLNs with dense layers (IMDb MLN, Accident MLN), it can be observed that CE-OR saves the computational costs as compared to C-SG-OR, significantly}. 


==> texFiles/extendedAbstract.tex <==
Graphs (or networks) are a natural way to analyze inter-related set of entities. When these entities are associated with a diverse number of features, each denoting a specific perspective, then the representation can be extended to form network of layers (one for each feature), known as multiplexes. For example, a set of people can be connected to each other via a number of different platforms like Facebook, LinkedIn, emails and so on. Therefore, in this case, the set of people, represented by nodes, will be connected by an edge depending on whether or not they are friends on Facebook, connections on LinkedIn or exchange emails, giving rise to multiple layers each highlighting a different interaction based perspective among the same set of people. Interesting insights into a multiplex can be obtained by analyzing the most tightly knit groups of entities (communities), the most influential entities (hubs or high centrality nodes), etc. Such analysis can be performed either layer-wise or by combining multiple layers. But, as the number of layers increases, holistic analysis of multiplexes by combining features in various ways can become challenging as well as computationally expensive. 

In a multiplex with N layers, a subset of layers can be chosen in $O(2^N)$ ways for combining. But, here the questions arises of how to combine any subset of layers. In this regard, our earlier work proposes the combination of multiplex layers using Boolean operations - AND, OR, NOT. 



In this paper, we address the task of efficiently composing entity communities for any combination of features (or multiplex layers) involving conjunction (AND), disjunction (OR) and negation (NOT) Boolean operations. A community is a group of tightly connected entities denoting that the entities in it are strongly similar. In this paper, we have demonstrated that a process based on set algebra can \textit{reconstruct} communities for any OR-Composed network. Apart from that, we have extended our earlier work (\cite{ICCS/SantraBC17} ) that highlighted the reconstruction of communities for any AND-Composed layer to work even with communities that are not self-preserving. Moreover, in order to support the processing of any random Boolean composition of multiplex layers, we have taken into consideration the communities of a NOT-composed layer. Our approach, when applied to real-world, multi-feature datasets such as IMDb (Internet Movie Database), DBLP (Database bibliography), traffic accidents and storms, show that we can reduce the overall space and time required to find communities in multiplexes while guaranteeing highly accurate reconstructed communities.

In this paper, for community-based analysis, we have proposed a cost-effective and elegant approach to combine results from multiple layers, without reconstructing the combined layers. Use of multiplexes (to divide the feature set)  makes it also easier to update, process, and understand information at individual layers. We therefore believe that the composition technique proposed here makes an important contribution to the nascent yet fast growing area of analyzing multiplexes.

The proposal should include: Topic, Key concepts, Methods, Expected Results and Conclusions. Please ensure that you include your full name and email contact details.  


==> texFiles/old-related_work.tex <==
\section{Related Work}
\label{sec:relatedWork}

We provide an overview of some of the related work including work in %data fusion, 
multilayer networks and community detection.

%{\bf Data Fusion:} The area of data fusion concerns combining different types of data from multiple sources to gain a holistic understanding of the situation. The main challenges in achieving high level information fusion \cite{blasch2012high} is to link information over different collections so that user queries can be answered based on information extracted from images, videos, and correlated with other sources. Identifying patterns is also relevant to understand frauds, money-laundering, terrorist activities etc. To the best of our knowledge, multiplexes and composition-based approaches have not been used for fusion. We believe that multiplex-based approaches can be beneficially used to fuse and analyze data with multiple features obtained from multiple sources. 

{\bf Multiplexes or Multilayer Networks:} Recently, significant amount of work has been done in the area of multilayer networks~\cite{MultiLayerSurveyKivelaABGMP13,Boccaletti20141} to handle varying interactions among the same set of entities such as co-authorship relationship in different conferences \cite{MinSubMulLayer2012}, citation relationship across different topics \cite{ng2011multirank}, interaction relationships based on calls/bluetooth scans \cite{ClusSpectral2011} and connection relationships across different social media platforms \cite{magnani2013formation}. Most of the work have tried to figure out \textit{overall multiplex diagnostics} such as degrees and distances by considering the multiplex layers \textit{individually}.

However, in order to understand the effect of multiple features using composition of individual multiplex layers, we need a principled approach to arbitrarily combine features (or layers) without having to construct combined layers and analyze them. This paper proposes such an approach for disjunctively composing any subset of multiplex layers without reconstruction. This approach significantly reduces the overall storage as well as cost of constructing composed layers and then analyzing them. Comparison with certain multiplex representation schemes such as adjacency tensors\cite{de2013mathematical,maruhashi2011multiaspectforensics} will not be appropriate with this work as computations based on any subset of layers will require the loading of the entire multiplex tensor, thus increasing the computational complexity in case of sparse networks. 

\textbf{Community Detection} is a well-studied problem in monoplex (single network) analysis. It involves identifying groups of vertices that are more connected to each other than to other vertices in the network. This objective is often translated into the problem of optimizing network parameters such as modularity ~\cite{Clauset2004} or conductance ~\cite{Leskovec08}. The combinatorial optimization problems for community detection are NP-complete ~\cite{Brandes03}.  A large number of competitive approximation algorithms exist (see reviews in %~\cite{porter09,
\cite{Fortunato2009, Xie2013}). Algorithms for community detection have been developed for a wide range of inputs including directed 
%Leicht08
~\cite{Yang10}, weighted 
%,Berry2011
~\cite{Liu2011}, and dynamic networks
%,Tantipathananandh2007,Thai2011, Bansal2011,
~\cite{porterchaos13}.  Recently there have also been algorithms for identifying overlapping communities
%Yang2013acm,
~\cite{Chakraborty2015a}. Parallel algorithms on different platforms (distributed, shared memory, GPU and MapReduce) have also been implemented
%,RiedyMEB12,BaderM08, Soman11
~\cite{StaudtSM14,BhowmickSrinivasan13}.

Recent work has also extended community detection algorithms for multilayer networks based on matrix factorization \cite{dong2012clustering, qi2012community}, pattern mining \cite{zeng2006coherent,silva2012mining},  cluster expansion philosophy \cite{li2008scalable} and Bayesian probabilistic models \cite{xu2012model}. In general, community detection involves finding groups of tightly connected vertices in a network ~\cite{CommFortunatoC09,CommNewGir04}. In this work, our focus is on composition of communities belonging to different layers in a lossless manner. We use already developed software for community detection. 
To the best of our knowledge, the problem of \textit{inferring the communities of the combined network from communities of individual layers has not been addressed earlier}.
